Understanding Video-Ad Consumption on YouTube: A Measurement Study on User Behavior, Popularity, and Content Properties

Faced with the challenge of attracting user attention and revenue, social media websites have turned to video advertisements (video-ads). While in traditional media the video-ad market is mostly based on an interaction between content providers and marketers, the use of video-ads in social media has enabled a more complex interaction, that also includes content creator and viewer preferences. To better understand this novel setting, we present the first data-driven analysis of video-ad exhibitions on YouTube.

==> todo.tex <==
\onecolumn
\begin{verbatim}
TODOS Paper: Understanding How Users Consume YouTube VideoAds

Data
----

    1. Dados dos watchs do YouTube (sendo executado)
    2. Gerar um tsv estilo o de Ad-Watchs


Perguntas Artigo
----------------
    Section 1: Intro
    Section 2: RW

    Section 3: Dataset
        Q1: VideoAd exhibition rate
        Q2: Skip Rate
        Q3: Watch in full rate

    Q1, Q2 and Q3 are described in our dataset section. Used in the rest of the 
    paper. 

    Section 4: VideoAd Popularity
        Q4. How popular are video ads inside the campus?
        Q5. How about global video ads popularity?
        Q6. How early do video ads become popular (inside and outside campus)?

    Q4, Q5 e Q6 are used to provide insights on the the length and popularity
    of ad campaigns. We can measure popularity in #views and watch_time for all
    three questions. 

    Section 5: Content Analysis
        Q7: Is there a correlation with video-popularity and ad-popularity? Probably yes
        Q8: How about if we compute an average per user (average ad-watch time)?
        Q9: Is there any correlation between video content and ad-content? Can
            be measured using the category or freebase topics.
    
    Q7, Q8 e Q9: Analyze the correlations between ad-content and video-content. It will
    be inetersting if some contents have more views. 

    Section 6: User Behavior
        Q10: Are there users that watch more ads?
        Q11: If a user is re-exposed to the same ad, will the view-length increase?

    Section 7: Conclusões

Plots Artigo
------------

    Q1: Number
    Q2: Number
    Q3: Number

    Q4-Q5-Q6: Fazer para dentro e fora do campus

    Q4: CCDF (loglog) - Fazer para watchtime e views
    Q5: CCDF (loglog) - Fazer para watchtime e views
    Q6: Scatter plot of Gini and Pop (watchtime ou views). 
        Pode ficar por último. O Gini mensura se a popularidade é
        concentrada em algumas janelas. Com sorte, vamos ver alguns grupos
        no scatter (popular concentrado e popular disperso)
    
    Q7: Scatter plot (video_pop, ad_pop). Fazer para base global (jsons) e 
    base da UFMG (popularidade no campus). Fazer para watch_time e views
    Q8: Scatter plot também. Contrastar com Q7. 
    
    Q9a: Popularidade das ads por categoria (dentro e fora do campus)
    Q9b: Popularidade por FreeBase topics (coletado no json), mais focado 
    Q9c: MutualInformation, ou InformationGain, ou ChiSq entre categoria da ad e do video.

    Q10: CCDF do watchtime per user. Cada ponto é a média de tempo visto de uma ad por um IP.
    Q11: Percentual da média de tempo visto para cada exposição. Média entre todos os usuários.
    Provavelmente temos que fazer com uma fração (100% da ad watched).

\end{verbatim}

